Approximations to worst-case data dropping: unmasking failure modes

A data analyst might worry about generalization if dropping a very small fraction of data points from a study could change its substantive conclusions. Checking this non-robustness directly poses a combinatorial optimization problem and is intractable even for simple models and moderate data sizes. Recently various authors have proposed a diverse set of approximations to detect this non-robustness. In the present work, we show that, even in a setting as simple as ordinary least squares (OLS) linear regression, many of these approximations can fail to detect (true) non-robustness in realistic data arrangements. We focus on OLS in the present work due its widespread use and since some approximations work only for OLS. Across our synthetic and real-world data sets, we find that a simple recursive greedy algorithm is the sole algorithm that does not fail any of our tests and also that it can be orders of magnitude faster to run than some competitors.

==> new_sections/abstract.tex <==
A data analyst might worry about generalization if dropping a very small fraction of data points from a study could change its substantive conclusions. Checking this non-robustness directly poses a combinatorial optimization problem and is intractable even for simple models and moderate data sizes.
Recently various authors have proposed a diverse set of approximations to detect this non-robustness. In the present work, we show that, even in a setting as simple as ordinary least squares (OLS) linear regression, many of these approximations can fail to detect (true) non-robustness in realistic data arrangements. We focus on OLS in the present work due its widespread use and since some approximations work only for OLS. \revision{Across our synthetic and real-world data sets, we find that a simple recursive greedy algorithm is the sole algorithm that does not fail any of our tests and also that it can be orders of magnitude faster to run than some competitors.}

%Of the approximations that do not fail our tests, we find not only that a simple recursive greedy algorithm is the most conceptually straightforward but also that it can be orders of magnitude faster to run than the others.
%Finding the worst-case data subset to drop poses a combinatorial optimization problem. To overcome this intractability, recent works propose using additive approximations, which treat the contribution of a collection of data points as the sum of their individual contributions, and greedy approximations, which iteratively select the point with the highest impact to drop and re-run the data analysis without that point \citep{broderick2023automatic,kuschnig2021hidden}. We identify that, even in a setting as simple as OLS linear regression, many of these approximations can break down in realistic data arrangements. Several of our examples reflect masking, where one data point may hide or conceal the effect of another data point. We provide recommendations for users and suggest directions for future development.

%A data analyst might worry about generalization if dropping a very small fraction of data points from a study could change its substantive conclusions. Finding the worst-case data subset to drop poses a combinatorial optimization problem. To overcome this intractability, \citet{broderick2023automatic}  pose a gradient-based approximation that takes derivatives in an instantiated weight space. Building on work where the dropped data subset is known in advance, we propose an alternative approximation using derivatives in parameter space. Both approximations treat the impact of a collection of data points as the sum of their individual contributions. We focus on a subset of linear regression analyses, where our proposed approximation reduces to that of \citet{kuschnig2021hidden}. We identify failure modes of both approximations. Many of our examples reflect ``masking,'' where data points may meaningfully affect a conclusion jointly but not individually. Finally, we suggest directions for future improvements.


%A data analyst might worry about generalization if dropping a very small fraction of data points from a study could change its substantive conclusions. Finding the worst-case data subset to drop poses a combinatorial optimization problem. \citet{broderick2023automatic} recently suggested to approximate the objective by instantiating continuous data weights and taking derivatives with respect to these weights; they show that the resulting optimization problem is fast to solve and can identify conclusion-changing small data subsets in influential real-life data analyses. \citet{kuschnig2021hidden} proposes other approximations based on derivatives in the parameter space. Focusing on certain data analyses using linear regression, we identify failure modes of all of these approximations. Many of our examples reflect ``masking,'' where data points may meaningfully affect a conclusion jointly but not individually. Our work suggests directions for future improvements.
